Towards 3D Molecule-Text Interpretation in Language Models

Language Models (LMs) have greatly influenced diverse domains. However, their inherent limitation in comprehending 3D molecular structures has considerably constrained their potential in the biomolecular domain. To bridge this gap, we focus on 3D molecule-text interpretation, and propose 3D-MoLM: 3D-Molecular Language Modeling. Specifically, 3D-MoLM enables an LM to interpret and analyze 3D molecules by equipping the LM with a 3D molecular encoder. This integration is achieved by a 3D molecule-text projector, bridging the 3D molecular encoder's representation space and the LM's input space. Moreover, to enhance 3D-MoLM's ability of cross-modal molecular understanding and instruction following, we meticulously curated a 3D molecule-centric instruction tuning dataset -- 3D-MoIT. Through 3D molecule-text alignment and 3D molecule-centric instruction tuning, 3D-MoLM establishes an integration of 3D molecular encoder and LM. It significantly surpasses existing baselines on downstream tasks, including molecule-text retrieval, molecule captioning, and more challenging open-text molecular QA tasks, especially focusing on 3D-dependent properties. We release our codes and datasets at https://github.com/lsh0520/3D-MoLM.

==> chapters/1_intro.tex <==
\section{Introduction}
The advent of Language Models (LMs) \citep{gpt3,gpt4,T5,bert,LLaMA, vicuna} has triggered a series of remarkable innovations across multiple disciplines, notably molecular understanding.
Recent works have explored aligning molecule data (\ie 1D sequences  \citep{scibert, kvplm, molt5, galactica} and 2D graphs \citep{momu, stm}) with LMs for a new generation of molecular LMs with strengthened ability to understand and reason about molecule structures.

However, prior works are not grounded in the 3D molecular world, which involves rich spatial geometric intricacies.
Specifically, 3D molecular coordinates convey crucial information to interpret molecular dynamics, protein-ligand interactions, enzymatic functions, and a host of other biomolecular phenomena \citep{3d-molecule-1, 3d-molecule-2}.
Point clouds \citep{point-cloud-review}, as a universal and efficient representation in 3D world, offer a promising solution for 3D molecule modeling.
Yet, despite it showcases advantages in conventional property prediction \citep{uni-mol} and molecular generation \citep{edm} tasks, \zhiyuan{3D-text interpretation is undefined} 3D-text interpretation is largely unexplored in molecules, \zhiyuan{the following sentence is grammarcally incorrect} but our focus in this paper.


\zhiyuan{Need to discuss related works first to support your argument that these three components are crucial.}
Towards effective 3D-text interpretation in LMs, we argue that three components are of crucial importance: (1) \zhiyuan{I thought we have decided to mention dataset as a main contribution}3D-text molecular pairs, \zhiyuan{as $\rightarrow$ which is} as the prerequisite to train a cross-modal LM with 3D-text interpretation ability, (2) \zhiyuan{cross-modal alignment is proposed by previous works, need citation to give them credit and support your argument  }cross-modal alignment, to establish a \zhiyuan{remove coarse-grained}coarse-grained connection between 3D molecular point clouds and corresponding texts, and (3) \zhiyuan{3D molecule-oriented instruction tuning} 3D instruction tuning, on properties closely related to molecular 3D conformations, to precisely activate the 3D perception and textual interpretation ability of the model.
Yet, existing works have not shown such tailor-made design for 3D-text interpretation.
\zhiyuan{Previous works~\cite{momu, stm}} MoMu \citep{momu} and MoleculeSTM \citep{stm} fuse the representations of 2D molecular graphs and texts through contrastive learning, without 3D perception to capture spatial information and instruct tuning for open-text QA.
Mol-Instructions \citep{mol-ins} provides molecular
instructions to tune a molecular LM, \zhiyuan{however is limited by the inability of perceiving 3D molecules}however with limited perception of 1D SELFIES \citep{selfies}.

% Specifically, molecular properties are associated mostly with their atomic composition, topological structure, and spatial coordinates. 
% However, the 1D sequence (\eg IUPAC name \citep{iupac}, SMILES \citep{smiles} and SELFIES \citep{selfies} string) and 2D graph of a molecule can only capture the first two aspects, ignoring spatial information.
% Consequently, existing models are still less than optimal to infer crucial properties that are closely related to 3D conformations (\eg the HOMO-LUMO Gap \citep{homo-lumo-gap} and SCF energy \citep{scf}) and the potential of LMs has not been fully realized in the complex world of biomolecular research.

To bridge this gap, we propose a \underline{3D} \underline{M}olecular \underline{L}anguage \underline{M}odel, \textbf{3D-MLM}, designed to bolster LM's molecular 3D-text interpretation by integrating a 3D molecular perceptor to encode 3D molecular point clouds with atomic features and spatial coordinates.
Specifically, 3D-MLM addresses aforementioned three challenges as follows.

% We draw inspiration from vision-language paradigms by employing a cross-modal projector, Q-Former \citep{blip2, instructblip}, to convert 3D molecular representations into 1D soft prompts within the LM's input space.
% This 3D insight amplifies the LM's ability to correlate intricate 3D conformations with molecular properties. 

\zhiyuan{I thought we have decided to not use dataset as a main contribution. In my opionion, usnig RDKit to synthesis conformation is not a contribution. Distilling knowledge from GPT can possibly be a contribution, since we have , however the following paragraph does not give enough attention to that part.}
\textbf{3D-text data acquisition.}
In the molecular realm, a high-quality 3D-text benchmark dataset is still absent.
Thus, we first collect 324k molecules with their SMILES and textual descriptions in PubChem \citep{pubchem}.
Subsequently, we leverage RDKit \citep{rdkit} to generate 3D molecular geometries based on SMILES, giving us 3D molecular point clouds with atomic types and raw coordinates. 
And for descriptive texts, the majority of collected texts lack sufficient documentation of their physical, chemical, or structural properties. 
Such a lack of comprehensiveness hinders LMs from achieving a thorough understanding.
Thus, we are motivated to scrupulously extract knowledge from GPT \citep{gpt3} to further elaborate these less informative texts. 
Consequently, we construct a 3D-text molecular dataset with over 300k 3D point clouds paired with informative descriptions.

\textbf{Cross-modal alignment.}
With 3D-text molecule pairs in hand, we draw inspiration from vision-language paradigms by employing a cross-modal projector, Q-Former \citep{blip2, instructblip}, to align 3D molecular representations with the LM's input space.
Concretely, to hone the alignment capability, the training of the cross-modal projector consists of two stages.
In the initial stage, both the projector and 3D molecular perceptor are optimized to distill molecule features most related to the text, granting the model robust molecule-text retrieval prowess.
In the subsequent stage, the cross-modal projector
is tethered to the LM and trained on molecule captioning.
This compels the projector to generate soft prompts seamlessly interpretable by the LM.
Such cross-modal alignment bridges the gap between the spaces of 3D molecular point clouds and language texts.

\textbf{3D instruction tuning.}
As the raw conformation generated by RDKit is inaccurate, it may be suitable for coarse-grain alignment \citep{blip,uni-mol}, but when facing fine-grained 3D-text interpretation, more precise spatial information are required.  
Meanwhile, the texts in alignment training are rather general descriptions (\eg molecular formula, weight and solubility) and lack specific knowledge related to the 3D spatial coordinates. 
Such texts pale when precisely and effectively activating the model's 3D perception.
Thus, We consider PubChemQC \citep{pubchemqc, molecule3d} as the source to collect accurate calculation of 3D geometries by DFT and quantitative properties closely related to molecular 3D conformations (\ie HOMO, LUMO and SCF energy). 
Subsequently, together with the textual descriptions for alignment, these data are transformed into instruct-tuning format \citep{ChatGPT} to perform fine-grained 3D-text interpretation.
And this 3D instruction tuning amplifies the LM's ability of correlating intricate 3D conformations with molecular properties and dealing with 3D molecular open-text QA. 

% To perform fine-grained 3D-text interpretation, we transform these data into instruct-tuning format \citep{instructgpt} 

% Meanwhile, molecule captioning task cannot endow the model with open-text QA capability.
% 3D-MLM tackles these two obstacles together by further performing 3D instruction tuning.

% Then, together with the textual descriptions for alignment, they are transformed into instruct-tuning format \citep{instructgpt}.


Experiment results show that (1) 3D-MLM significantly outperforms existing molecular cross-modal models on cross-modal retrieval and molecule captioning, demonstrating the effectiveness of Q-Former to connect the 3D molecular graph and textual representation space. (2) 
3D-MLM surpasses the baseline LMs without 3D molecular perception on open-text QA tasks, especially on properties closely related to 3D spatial information (\ie HOMO, LUMO and SCF energy), verifying its capability of 3D-text interpretation.


% Experiment results indicate that our PointLLM demonstrates substantially better performance over 2D baselines,
% and in over 50\% of tested samples of object captioning, it
% gains higher scores than human annotators in human evaluation. To supplement these quantitative evaluations, we also
% present a range of qualitative examples, offering a broader
% perspective on our model’s real-world performance.

% The next challenge resides in how to precisely activate the 3D perception capability of the model.
% Concretely, the texts elaborated by GPT contain rather general descriptions and lacks specific knowledge related to the 3D spatial coordinates of molecules. 
% Thus it may be adequate for coarse-grained alignment, but cannot precisely activate the model's 3D perception capability.
% Motivated by this, we continue to collect quantitative properties closely related to molecular 3D conformations (\ie HOMO, LUMO and SCF energy) from PubChemQC \citep{pubchemqc} and transform them into instruct-tuning format \citep{instructgpt}.

% We demonstrate (1) the effectiveness of Q-Former to bridge the 3D molecular graph and textual representation space by cross-modal retrieval and graph-based molecule captioning tasks, and (2) the superiority of MolGLA through the performance on cross-modal descriptive and computational property QA datasets.



==> chapters/backup/0_abstract.tex <==
% \begin{abstract}
%     Language Models (LMs) have catalyzed significant advancements across a spectrum of fields. 
%     However, their proficiency within biomolecular domain remains limited due to an inherent limitation -- 3D geometrical perception, which is a critical ability of human professionals in comprehending molecular structures. 
%     To bridge this gap, we propose \textbf{MolGLA}: \underline{Mol}ecular \underline{G}raph-\underline{La}nguage model, which enhances an LM (\ie Vicuna) of only 1D text perception with a 3D molecular graph perceptor (\ie Uni-Mol) via the cross-modal projector.
%     Additionally, to establish effective connection between the molecular graph and text space, and augment the molecular knowledge with the cross-modal understanding, we meticulously curated cross-modal molecular graph-text alignment and instruction QA datasets for MolGLA.
%     Specifically, MolGLA performs two stages training: (1) pretraining on molecular graph-text alignment dataset to activate its cross-modal projector, and (2) instruction tuning on molecular QA dataset to boost its cross-modal understanding and molecular inference ability. 
%     To showcase its effectiveness, we extensively benchmark MolCA on tasks of molecule-text retrieval, molecular captioning and more challenging descriptive and computational property QA, on which MolCA significantly outperforms the baselines.
% \end{abstract}
\begin{abstract}
    Language Models (LMs) have revolutionized a spectrum of fields, yet their potential in the biomolecular domain is constrained by the absence of 3D geometric understanding. 
    This capability is vital for chemical experts analyzing molecular structures and properties. 
    To address this challenge, we propose \textbf{MolGLA}: \underline{Mol}ecular \underline{G}raph-\underline{La}nguage model, which enhances an LM (\ie Vicuna) of only 1D text perception with a 3D molecular graph perceptor (\ie Uni-Mol) via a cross-modal projector bridging their representation spaces. 
    Additionally, to establish effective connection between the molecular graph and text space, and augment the molecular knowledge with the cross-modal understanding, we meticulously curated cross-modal molecular graph-text alignment and instruction QA datasets for MolGLA.
    Specifically, MolGLA's training involves: (1) pretraining on the alignment dataset to activate its cross-modal projector, and (2) instruction fine-tuning to enhance its molecular understanding. 
    Our evaluations on molecule-text retrieval, molecular captioning, and more challenging  descriptive and computational property QA tasks indicate that MolGLA significantly surpasses existing benchmarks.
\end{abstract}

==> chapters/backup/1_intro.tex <==
\section{Introduction}
The advent of Language Models (LMs) \citep{gpt3,gpt4,T5,bert,LLaMA, vicuna} has triggered a series of remarkable innovations across multiple disciplines. 
Meanwhile, extensive human-curated biochemical knowledge, represented in textual format, captures the intricate properties of molecules. 
Such textual training corpus further deepens the molecular comprehension of LMs \citep{scibert, kvplm, molt5, galactica}, bolstering their capacity to aid in biochemical research.

Conventional LMs, as depicted in Figure 1(a), are designed to handle 1D sequential data, leading them to represent molecules using their 1D Simplified Molecular Input Line Entry System (SMILES) strings \citep{smiles} and process them akin to regular texts.
This design, with text-bound processing, confines their capabilities when introduced to the complex world of biomolecular research, which necessitates a deep grasp of molecules' 3D geometric intricacies — an aspect crucial for decoding molecular dynamics, protein-ligand interactions, enzymatic functions, and a host of other biomolecular phenomena \citep{3d-molecule-1, 3d-molecule-2}.
For example, cis and trans isomers may exhibit different reactivities with certain reagents or under specific conditions because of the spatial arrangement of their functional groups. In essence, spatial differences can influence reactivity \citep{chem-textbook}.

To address this, recent studies \citep{momu,stm} integrate 2D molecular graphs into LMs using cross-modal contrastive learning \citep{clip,declip}, as depicted in Figure 1b. 
Such an approach aligns the graph representations generated by the graph encoder with textual representations derived from the LM, allowing the LM to understand the topological structure of molecular graphs.
Yet, we reveal the limitations of existing works from three perspectives:
\begin{itemize}[leftmargin=*]
    % \item A close examination of leading vision-language cross-modal pretraining frameworks \cite{clip,blip} reveals that achieving superior multi-modal alignment necessitates extensive cross-modal data pairs. 
    % In the molecular realm, however, a large-scale multi-modal benchmark dataset, offering comprehensive textual descriptions covering structural characteristics and chemical-physical properties, is still absent.
    \item Representing a molecule with just a 2D graph constrains the model's molecular comprehension. 
    Certain chemical properties of molecules (\eg free energy and the HOMO-LUMO gap \citep{homo-lumo-gap}) are derived from 3D equilibrium conformations, which have a notable difference from 2D molecular graphs. 
    Since the design of new materials and molecules in computational methods relies heavily on these properties, using 2D graphs for molecular representation could be inadequate.
    \item Existing works leverage contrastive learning for cross-modal representation fusion, which is not naturally adaptable for tasks like open-ended molecule-to-text generation.
    Concretely, it aims to align representations from distinct uni-modal encoders, such as those for molecular graphs and texts.
    However, molecule-to-text task demands LMs to interpret molecular graphs as inputs, a requirement contrastive learning isn't inherently equipped for, thus underutilizing the potential of prevailing large LMs with decoder-only structure \citep{LLaMA, llama2, vicuna}.
\end{itemize}

To bridge this gap, we propose a \underline{Mol}ecular \underline{G}raph-\underline{La}nguage model, \textbf{MolGLA}, designed to bolster the molecular comprehension of an LM (\ie Vicuna \citep{vicuna}) by integrating a 3D molecular graph perceptor (\ie Uni-Mol \citep{uni-mol}).
Specifically, we draw inspiration from vision-language paradigms by employing a cross-modal projector, Q-Former \citep{blip2, instructblip}, to convert 3D molecular graph representations into 1D soft prompts within the LM's input space.
This 3D insight amplifies the LM's ability to correlate intricate 3D conformations with molecular properties. 
However, leading vision-language cross-modal pretraining frameworks \citep{clip,blip} reveal that achieving high-quality cross-modal alignment between representation spaces necessitates extensive cross-modal data pairs. 
Yet, in the molecular realm, a large-scale multi-modal benchmark dataset, offering comprehensive textual descriptions covering structural characteristics and chemical-physical properties, is still absent.

To tackle this, we construct a cross-modal molecular graph-text dataset, \textbf{MolPubChem}, which first collects molecules with their corresponding textual descriptions in PubChem \citep{pubchem}. 
Despite the plethora of molecules identified in PubChem, the majority lack sufficient documentation of their physical, chemical, or structural properties. 
Such lack of comprehensiveness hinders LMs from achieving a thorough understanding.
Thus, we are motivated to scrupulously extract knowledge from GPT \citep{gpt3} to further polish these less informative texts. 
This helps to harness the power of LMs by establishing a strong connection between molecular structure and properties,thus benefiting downstream tasks of molecular understanding.

As depicted in the Figure, MolGLA employs a tri-phase training approach.
The initial two stages focus on honing the cross-modal projector's alignment capabilities. 
During the first stage, both the projector and graph encoder are optimized to distill molecule features most related to the text, granting the model robust molecule-text retrieval prowess. 
In the subsequent stage, the cross-modal projector is tethered to a frozen LM and trained on molecule captioning. 
This compels the projector to generate soft prompts seamlessly interpretable by the LM. 
In the culmination stage, MolGLA undergoes instruction fine-tuning on a cross-modal QA dataset, amplifying its molecular comprehension.

We demonstrate (1) the effectiveness of Q-Former to bridge the 3D molecular graph and textual representation space by cross-modal retrieval and graph-based molecule captioning tasks, and (2) the superiority of MolGLA through the performance on cross-modal descriptive and computational property QA datasets.



==> chapters/backup/2_related.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{charts/related_work.pdf}
    % \vspace{4pt}
    \caption{
    \lsh{(a) Illustration of molecular graph and language model.
    (b) Evaluation of the correctness and comprehensiveness of MoLa-D and MoLa-(s)D by three chemical experts and GPT-4.}
    }  
    \label{fig:related_work}
    \vspace{-12pt}
\end{figure}
\section{Related Work}
\subsection{Molecular Language Models}
General LMs \citep{gpt3,gpt4, LLaMA}, especially large LMs, have acquired some biochemistry-related knowledge from vast amounts of training corpus.
Subsequently, to enhance the molecular understanding, a large amount of scientific papers are added to the training corpus, giving us more scientific LMs.
Specifically, built upon BERT \citep{bert}, Sci-BERT \citep{scibert} leverages unsupervised pretraining on a large multi-domain corpus of scientific publications.
To dive deeper into molecular modeling, KV-PLM \citep{kvplm} extends the tokenizer in Sci-BERT to incorporate molecule knowledge from versatile reading on both molecule structure (\ie SMILES string) and biomedical text information.
And based on T5 \citep{T5}, MolT5 \citep{molt5} is trained by translation between molecular SMILES and textual descriptions.
Recently, Meta introduces Galactica \citep{galactica}, which is trained on a highly curated corpus that includes scientific articles, patents, and databases. 
As depicted in Figure \ref{fig:related_work}(a), aforementioned LMs extract knowledge from one-dimensional sequence such as names, SMILES strings, and textual descriptions of molecules, which falls short in providing sufficient structural information to infer physical, chemical, and biological properties.

\subsection{Molecular Graph-Language Models}
Inspired by multi-modal representation alignment \citep{clip,declip}, researchers \citep{momu,stm} incorporate topological understanding into LMs through contrastive pre-training using pairs of molecular graphs and corresponding texts.
From data perspective, high-quality and large-scale graph-text pairs is the prerequisite for effective alignment.
\lsh{MoMu \citep{momu} collects 15K molecular graphs with their corresponding documents from PubChem and S2orc \citep{s2orc} to form a multi-modal molecular dataset. 
And MoleculeSTM \citep{stm} constructs a dataset with over 280K molecular graph-text pairs from PubChem.
Nevertheless, as shown in Figure \ref{fig:related_work}(b), the majority of textual descriptions for molecules in PubChem do not offer comprehensive contexts that encompass structural features, chemical, and physical properties, resulting in a lack of thoroughness.}
% Nevertheless, aside from their small scales, the textual descriptions in existing open-source molecular multi-modal datasets have either low signal-noise-ratio \citep{momu} or information density \citep{kvplm, molt5} (see Figure \ref{fig:related_work}(b) for examples), which motivates us to construct a dataset with larger scale and more comprehensiveness.
Meanwhile, from model perspective, the contrastive pretraining pulls close the same molecule' graph and textual representations, and pushes those of different molecules away from each other.
Such alignment implicitly fuse representations of diverse modalities as in Figure \ref{fig:related_work}(a).
Yet, we reveal two limitations for such simple alignment: (1) implicit alignment may not be sufficient for effective cross-modal information fusion, and (2) the encoder-only architecture may not be readily transferable to diverse downstream tasks, particularly those involving complex generation tasks.
And this motivates us to go beyond cross-modal representation alignment and devise a versatile framework to fulfill the potential for both encoding and decoding tasks.

==> chapters/backup/4_method.tex <==
\section{MoLa: Molecular Graph-Language Pretraining Framework}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{charts/framework.pdf}
    \caption{Versatile model architecture and multi-task pretraining strategy of MoLa (blocks with the same color share the same parameters and gradient back-propagation is stopped along dashed paths). 
    It has multiple encoding and decoding structures, making it adaptable to various molecular understanding and generation tasks.}
    \label{fig:framework}
    \vspace{-8pt}
\end{figure}
The core idea of MoLa is the integration and alignment of molecular graphs and textual descriptions, which empowers the LM to have a multi-view of molecules for both graph- and text-centric knowledge.
Consequently, the model not only reads the 2D molecular graphs and understands the topological knowledge in chemistry, but also enables the graph-guided generation of the language description.

As shown in Figure \ref{fig:framework}, MoLa attains the graph-language alignment goal by operating three functionalities: uni-modal encoder, cross-modal encoder, and cross-modal decoder.
First, MoLa builds three uni-modal encoders to yield representations that distill text- and graph-centric knowledge.
Then, it transplants cross-attention blocks into the text encoder to accomplish the cross-modal information fusion.
MoLa next constructs a cross-modal decoder to translate the graph information into texts by replacing the self-attention blocks with causal self-attention blocks.
To activate these three functionalities, we devise multi-task pretraining objectives: uni-modal representation alignment, cross-modal pair matching, and graph-guided language modeling.

\subsection{Versatile Model Architecture}
We first outline the input format of MoLa.
Formally, let $(g,t)$ be a graph-text pair describing a molecule, where $g$ and $t$ are its 2D graph and associated textual description, respectively.
Furthermore, we expand each pair to a triplet $(g, s, t)$ by including its SMILE string $s$.
For graph modality, $g$ is represented as $(\Set{V},\Set{E},\Mat{x}_{g})$, where $\Set{V}$ and $\Set{E}$ separately denote the sets of atomic nodes and bond edges, and $\Mat{x}_{g}$ collects the features of all nodes and edges.
In the language modality, $s$ and $t$ are transformed into the sequences of $N$ and $M$ tokens, $\Mat{x}_{s}$ and $\Mat{x}_{t}$, respectively, by the tokenizer and word embedding layer.
Hence, we present distinct levels of a molecule, 2D graph and 1D sequence, as follows:
\begin{gather}\label{equ:graph-text-pair}
    g = (\Set{V},\Set{E},\Mat{x}_{g}),\quad \Mat{x}_{s} = [s_0, s_1, ..., s_{N-1}], \quad  \Mat{x}_{t} = [t_0, t_1, ..., t_{M-1}].
\end{gather}

\subsubsection{Uni-Modal Encoders}
We first build uni-modal encoders to separately encode the graphs and texts.
We note that the size of datasets (\ie 320K graph-text pairs) is relatively small compared to the peers from other domains (\eg 400M image-text pairs in CLIP \citep{clip}).
To alleviate the data insufficiency issue, encoders are initiated with the pretrained checkpoints for individual modalities.

\noindent\textbf{Graph Encoder.}
For graph representations, we adopt the pretrained GIN encoder \citep{gin} from GraphMVP \citep{graphmvp} as our graph encoder: $\text{GEncoder}(\cdot)$.
Upon graph $g$ with $|\Set{V}|$ nodes, it applies a graph neural network (GNN) which recursively propagates and aggregates information among nodes, to obtain the node-level representations $\Mat{h}_g \in \Space{R}^{|\Set{V}| \times d_g}$ and pool them into the graph-level representation $\Mat{z}_g \in \Space{R}^{1 \times d_g}$ with the hidden dimension of $d_g$.
Formally, the graph encoding procedure is as follows:
\begin{gather}\label{equ:graph-encoder}
    \Mat{z}_{g} := \text{GEncoder}(g)=\text{Pool}(\Mat{h}_{g}),\quad \Mat{h}_{g} = \text{GNN}(\Mat{x}_{g},g),
\end{gather}
where $\Mat{h}_{g}$ is the node representations yielded by the GNN and $\text{Pool}(\cdot)$ is the pooling function.

\noindent\textbf{Language Encoder.}
To encode both SMILES strings and textual descriptions of molecules, KV-PLM \citep{kvplm}, which are based on BERT \citep{bert}, is adopted as the SMILES and text encoders: $\text{SEncoder}(\cdot)$ and $\text{TEncoder}(\cdot)$.
Specifically, given the SMILES sequence $\Mat{x}_s$ in Equation \eqref{equ:graph-text-pair}, we first append a special token [SMI] to the beginning as the input sequence $\Mat{h}_s^0 \in \Space{R}^{(N+1) \times d_t}$, where $d_t$ is the hidden size.
On this input, $L$ transformer layers with self-attention (SA) and feed-forward network (FFN) blocks are employed to create $\Mat{h}_s^L \in \Space{R}^{(N+1) \times d_t}$ and pool them into the SMILES representation $\Mat{z}_s \in \Space{R}^{1\times d_t}$:
\begin{gather}\label{equ:smiles-encoder}
    \Mat{z}_{s} := \text{SEncoder}(\Mat{h}_{s}^0)=\text{Pool}(\Mat{h}_{s}^{L}),\quad \Mat{h}_{s}^l = \text{FFN}^l(\text{SA}^l(\Mat{h}_{s}^{l-1})),\quad \Mat{h}_{s}^0 = \text{Concate}(\text{[SMI]},\Mat{x}_s),
\end{gather}
where $\Mat{h}_{s}^l$ is the sequence representations derived from the $l$-th layer with $\text{FFN}^l(\cdot)$ and $\text{SA}^l(\cdot)$, $l\in\{1,\cdots,L\}$; $\text{Concate}(\cdot)$ is the concatenate function.

Analogously, we exploit the shared transformer layers to process the text sequence $\Mat{x}_t$ with a special token $\text{[CLS]}$ and get the textual representation $\Mat{z}_t \in \Space{R}^{1 \times d_t}$:
\begin{gather}\label{equ:text-encoder}
    \Mat{z}_{t} := \text{TEncoder}(\Mat{h}_{t}^0)=\text{Pool}(\Mat{h}_{t}^{L}),\quad \Mat{h}_{t}^l = \text{FFN}^l(\text{SA}^l(\Mat{h}_{t}^{l-1})),\quad \Mat{h}_{t}^0 = \text{Concate}(\text{[CLS]},\Mat{x}_t).
\end{gather}
% where $\Mat{h}_{t}^l$ is the sequence representations derived from the $l$-th layer with $\text{FFN}^l(\cdot)$ and $\text{SA}^l(\cdot)$, $l\in\{1,\cdots,L\}$; $\text{[CLS]}$ is a special token concatenated with $\Mat{x}_t$.

\subsubsection{Cross-Modal Encoder}
To explicitly fuse the topological knowledge and semantic information, we inject the graph representation into the language encoder, which alters to become the cross-modal encoder.
Specifically, a cross-attention (CA) block \citep{cross-att} is inserted between the SA and FFN blocks in each layer, enabling the cross-modal encoder $\text{CEncoder}(\cdot)$ to yield the cross-modal representation $\Mat{z}_c$ as follows:
\begin{align}\label{equ:cross-modal-encoder}
    \Mat{z}_c :=& \text{CEncoder}(\Mat{h}_c^0)=\text{Pool}(\Mat{h}_c^L),&\Mat{h}_c^l &= \text{FFN}^l(\text{CA}^{l}(\text{SA}^l(\Mat{h}_c^{l-1}), \hat{\Mat{z}})), \nonumber\\
    \hat{\Mat{z}}_g=&\text{Concate}(\Mat{z}_g,\Mat{h}_g),& \Mat{h}_c^0 &= \text{Concate}([\text{ENC}], \Mat{x}_{t}),
\end{align}
where $\hat{\Mat{z}}\in\Space{R}^{(2+|\Set{V}|)\times d_{g}}$ combines graph and SMILES representations from Equation \ref{equ:graph-encoder} \& \ref{equ:smiles-encoder}: $\Mat{z}_s$, $\Mat{z}_g$ and $\Mat{h}_g^{L}$, which depict both the global and local structures; [ENC] token is appended to the text sequence $\Mat{x}_t$ as the input;
$\Mat{h}_c^l$ is the sequence representations obtained from the $l$-th layer with $\text{FFN}^l(\cdot)$, $\text{CA}^{l}(\cdot)$, and $\text{SA}^l(\cdot)$.
Clearly, the CA blocks fuse the information across the graph and language modalities.

\subsubsection{Cross-Modal Decoder}
A versatile architecture is able to adapt to not only uni-modal or cross-modal understanding, but also generation tasks.
Thus, to equip MoLa with graph-based text generation ability, a cross-modal decoder is constructed by replacing the SA blocks in the cross-modal encoder with causal self-attention (C-SA) blocks, in which a causal attention mask restricts the self-attention mechanism to attend only to the previous positions in the input sequence.
Analogously, the processing procedure of the cross-modal decoder $\text{CDecoder}(\cdot)$ is formulated as:
\begin{gather}\label{equ:cross-modal-decoder}
    \Mat{z}_d := \text{CDecoder}(\Mat{h}_d^0)=\Mat{h}_d^L, \ \  \Mat{h}_d^l = \text{FFN}^l(\text{CA}^{l}(\text{C-SA}^l(\Mat{h}_d^{l-1}), \hat{\Mat{z}})), \ \  \Mat{h}_d^0 = \text{Concate}([\text{DEC}], \Mat{x}_t),
\end{gather}
where a $\text{[DEC]}$ token is added to indicate the beginning of the input textual sequence and $\Mat{z}_d \in \Space{R}^{(1+M) \times d_t}$ summarizes the representations of tokens for word prediction.
Consequently, the cross-modal decoder with causal attention mechanism could be adopted in generation tasks such as language modeling, where the goal is to predict the next word in a sequence based on the previous words.

Studies on vision-language pre-training \citep{albef,blip} have demonstrated that the discrepancies between the encoding and decoding tasks are most effectively captured by the SA and C-SA blocks, whereas the word embedding, CA, and FFN blocks are similar for both tasks. 
To enhance the model efficiency, as depicted in Figure \ref{fig:framework}, the language encoders and decoder in MoLa share most of their parameters, with the exception of the SA and C-SA blocks.

\subsection{Multi-Task Pretraining Objectives}
To activate multiple branches of MoLa, we devise a multi-task pretraining strategy, including uni-modal alignment, cross-modal pair matching, and graph-guided language modeling.

\textbf{Uni-Modal Representation Alignment.}
The graph representation $\Mat{z}_g$ in Equation \eqref{equ:graph-encoder} of a molecule embodies its topological and structural knowledge, while its textual representation $\Mat{z}_t$ in Equation \eqref{equ:text-encoder} portrays its high-level properties. 
Additionally, the training corpus of KV-PLM \citep{kvplm}, which furnishes the initialization weights for our text encoder, comprises SMILES strings, thereby indicating that the SMILES representation encapsulates molecule-related knowledge as well. 
Thus, we include its representation $\Mat{z}_s$ in the unimodal representation alignment as well.
Concretely, the representations of $\Mat{z}_g, \Mat{z}_s, \Mat{z}_t$ are projected to the same $d$-dimensional latent space $\Space{R}^{d}$ for pairwise contrast, giving us $\Tilde{\Mat{z}}_g, \Tilde{\Mat{z}}_s, \Tilde{\Mat{z}}_t$.
% Hereafter, InfoNCE \citep{infonce} is adopted as the contrastive loss $l_{\text{con}}$ to align the pairs of the same molecule and contrast those of different molecules simultaneously.
And the loss function of uni-modal representation alignment $\lapl_{\text{ali}}$ is formulated as:
\begin{equation}\label{equ:alignment-loss}
    \lapl_{\text{ali}} = \Space{E}_{(g, s, t)}( l_{\text{con}}(\Tilde{\Mat{z}}_g, \Tilde{\Mat{z}}_s) + l_{\text{con}}(\Tilde{\Mat{z}}_g, \Tilde{\Mat{z}}_t) + l_{\text{con}}(\Tilde{\Mat{z}}_s, \Tilde{\Mat{z}}_t)),
\end{equation}
% \begin{equation}\label{equ:alignment-loss-1}
%     \lapl_{\text{ali}} = \Space{E}_{(g, s, t)}( l_{\text{con}}(g, s) + l_{\text{con}}(g, t) + l_{\text{con}}(s, t)),
% \end{equation}
% \begin{equation}\label{equ:ali-loss-2}
% % \lapl_{\text{ali}} = \Space{E}_{(\Mat{h}_g, \Mat{h}_s, \Mat{h}_t)}( \lapl_{\text{InfoNCE}}(\Mat{h}_g, \Mat{h}_s) + \lapl_{\text{InfoNCE}}(\Mat{h}_g, \Mat{h}_t) + \lapl_{\text{InfoNCE}}(\Mat{h}_s, \Mat{h}_t)) \nonumber \\
%     l_{\text{con}}(g, t)=- 
%     (
%     \log{\frac{\text{exp}{(E(g, t))}}{\text{exp}{(E(g,t))} \mathpunct{+} \displaystyle \sum_{t'}\text{exp}{(E(g, t'))}}}
%     +
%     \log{\frac{\text{exp}{(E(g, t))}}{\text{exp}{(E(g, t))} \mathpunct{+} \displaystyle \sum_{g'}\text{exp}{(E(g', t))}}}
%     ),
% \end{equation}
where the contrastive loss $l_{\text{con}}$ is instantiated as InfoNCE loss \citep{infonce} to align the pairs of the same molecule and contrast those of different molecules simultaneously in batches.
% where function $E(g, t)=\Trans{||\Tilde{\Mat{z}}_g||}||\Tilde{\Mat{z}}_t||/\tau$ evaluates the cosine similarity between the graph representation $\Tilde{\Mat{z}}_g$ and text representation $\Tilde{\Mat{z}}_t$ with a temperature hyperparameter $\tau$; the negative graph $g'$ and text $t'$ are randomly sampled from the triplets of other molecules in the same minibatch and $l_{\text{con}}(g, s)$ and $l_{\text{con}}(s, t)$ can be obtained analogously.
Representation alignment enables MoLa to perform cross-modal retrieval task in downstream.

\textbf{Cross-Modal Pair Matching.}
Pair matching loss $\lapl_{mat}$ enforces the model to learn finer-grained graph-text cross-modal representations. 
Thus, we append a simple MLP-based matching head $r(\cdot)$ after the cross-modal encoder and design a simple binary classification task to predict whether a graph-text pair is positive (matched) or negative (unmatched) given its cross-modal representation $\Mat{z}_c$:
\begin{gather}\label{equ:pair-matching-loss}
    % \lapl_{\text{mat}} = -\Space{E}_{(g, t)}(y\text{log}(p)+(1-y)\text{log}(1-p)),\quad p=r(\Mat{z}_c)
    \lapl_{\text{mat}} = \Space{E}_{(g, t)}l_{CE}(p,y),\quad p=r(\Mat{z}_c)
\end{gather}
where $l_{CE}(\cdot)$ is the cross entropy loss, $y$ is the binary indicator if molecular graph $g$ matches with textual description $t$, and $p$ is the predicted probability of it.
Afterwards, this pair matching could be transplanted for text-guided molecule generation and editing (see Section \ref{sec:molecule generation and editing}).

\textbf{Graph-Guided Language Modeling.}
Language modeling loss $\lapl_{\text{lm}}$ aims to activate the cross-modal text decoder by training the model to maximize the likelihood of a word in the textual description based on graph representation and words in the front, which is instantiated as a cross entropy loss with a label smoothing rate of $0.1$:
\begin{gather}\label{equ:language-modeling-loss}
    \lapl_{\text{lm}} = \Space{E}_{(g, t)}l_{CE}(\hat{\Mat{x}}_d,\Mat{x}_t),\quad \hat{\Mat{x}}_d=f(\Mat{z}_d[:-1])=[\hat{t}_0,\hat{t}_1,...,\hat{t}_{M-1}],
\end{gather}
where $f(\cdot)$ is a classifier to decode the output $\Mat{z}_d$ in Equation \eqref{equ:cross-modal-decoder} into natural language.
It enables the model to convert molecular graphs into textual property descriptions (\ie molecule captioning).

Finally, the loss functions are jointly optimized: 
\begin{gather}\label{equ:overall-loss}
    \lapl=\lapl_{\text{ali}}+\lapl_{\text{mat}}+\lapl_{\text{lm}},
\end{gather}
% MoLa's multi-task pretraining strategy with uni-modal representation alignment, cross-modal pair matching, and graph-guided language modeling fulfills the potential for both molecular understanding and generation tasks in downstream.


==> chapters/backup/5_experiment_backup.tex <==
\section{Experiment}

\begin{table}[t]
\centering
\caption{Cross-modal retrieval results (\%) on the test-set of MolPubChem. \textbf{Bold} and \underline{underline} indicate the best and the second best performance, respectively.}
\begin{small}
\label{tab:cross-modal-retrieval}
\begin{tabular}{lcccccccc}
    \toprule
    & \multicolumn{4}{c}{Retrieval in batch} & \multicolumn{4}{c}{Retrieval in test set} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
    & \multicolumn{2}{c}{M2T (\%)} & \multicolumn{2}{c}{T2M (\%)} & \multicolumn{2}{c}{M2T (\%)} & \multicolumn{2}{c}{T2M (\%)} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    Model & Acc & R@20 & Acc & R@20 & Acc & R@20 & Acc & R@20 \\
    \midrule
   \multicolumn{2}{l}{\textbf{1D SMILES}} & & \multicolumn{1}{l}{} & & & \multicolumn{1}{l}{} & & \multicolumn{1}{l}{} \\
   Sci-BERT$^\dag$ & 83.28 & 97.68 & 84.02 & 97.41 & 71.85 & 85.48 & 72.26 & 84.71 \\
   KV-PLM$^\dag$ & 82.86 & 97.48 & 84.51 & 97.81 & 72.23 & 84.56 & 72.39 & 85.38 \\\midrule
   \multicolumn{2}{l}{\textbf{2D Graph}} & & \multicolumn{1}{l}{} & & & \multicolumn{1}{l}{} & & \multicolumn{1}{l}{} \\
   MoMu-S$^\dag$ & 90.82 & 98.27 & 90.12 & 98.35 & 78.44 & 93.08 & 78.98 & 92.97 \\
   MoMu-K$^\dag$ & 89.01 & 98.36 & 89.23 & 98.66 & 79.01 & 92.89 & 79.42 & 93.15 \\
   MoleculeSTM$^\star$ & 94.26 & 98.1 & 92.84 & 98.3 & 81.84 & 95.46 & 82.07 & 95.08 \\
   \midrule
   \multicolumn{2}{l}{\textbf{3D Graph}} & & \multicolumn{1}{l}{} & & & \multicolumn{1}{l}{} & & \multicolumn{1}{l}{} \\
   MolGLA w/o MTM & \underline{97.70} & \multicolumn{1}{c}{\underline{99.85}} & \underline{97.75} & \multicolumn{1}{c}{\underline{99.74}} & \multicolumn{1}{c}{\underline{84.86}} & \underline{98.47} & \multicolumn{1}{c}{\underline{84.81}} & \underline{98.62} \\
   3D-MoLM & \textbf{98.41} & \multicolumn{1}{c}{\textbf{99.95}} & \textbf{97.95} & \multicolumn{1}{c}{\textbf{99.95}} & \multicolumn{1}{c}{\textbf{87.16}} & \textbf{99.13} & \multicolumn{1}{c}{\textbf{84.81}} & \textbf{98.82} \\
   \bottomrule
   \end{tabular}
\end{small}
\end{table}

\begin{table*}[t]
\centering
\caption{Molecule captioning results (\%) on the test-set of MolPubChem. 
\textbf{Bold} and \underline{underline} indicate the best and the second best performance, respectively.
B-2: BLEU-2, B-4: BLEU-4, R-1: ROUGE-1, R-2: ROUGE-2, R-L: ROUGE-L, M: METEOR.}
% \begin{small}
\label{tab:molecule-captioning}
\begin{tabular}{lcccccc}
\toprule
Model & B-2 & B-4 & R-1 & R-2 & R-L & M \\
\midrule
\multicolumn{7}{l}{\textbf{1D SMILES}}  \\
MolT5-small &  20.53 & 13.23   & 28.44  & 11.45  & 18.30& 21.98 \\
MolT5-base  &  22.51 & 14.61 & 30.19  & 12.04 & 19.35  & 24.10 \\
MolT5-large  &  22.02 & 14.99 & 32.61  & 14.36 & 20.11  & \underline{24.74}\\
Llama2-7B  & 21.97 & 15.09 & \underline{33.76}  & 15.13 & 21.04  & 24.25
\\
\midrule
\multicolumn{7}{l}{\textbf{1D SMILES + 2D graph}}  \\
MoMu-small  &  21.08 & 13.58   & 28.33  & 11.34  & 18.32 & 21.89\\
MoMu-base   &  \underline{22.81} & 14.86 & 30.38  &12.19  & 19.45 & 24.11 \\
MoMu-large   &  22.20 & \underline{15.41} & 32.19 &\underline{14.63}  & \underline{20.18} & 24.59 \\
\midrule
\multicolumn{7}{l}{\textbf{1D SMILES + 3D structure}} \\
3D-MoLM        &  \textbf{24.56} & \textbf{16.83} & \textbf{37.45}  & \textbf{17.26}  & \textbf{23.52}  & \textbf{26.08} \\
\bottomrule
\end{tabular}
% \end{small}
\end{table*}

\begin{table*}[t]
\centering
\caption{QA results (\%) on the descriptive property subset of 3D-MoIT. 
\textbf{Bold} and \underline{underline} indicate the best and the second best performance, respectively. 
* denotes official checkpoint without instruct-tuning on 3D-MoIT.
% B-2: BLEU-2, B-4: BLEU-4, R-1: ROUGE-1, R-2: ROUGE-2, R-L: ROUGE-L, M: METEOR.
}
\label{tab:instruction-com}
\begin{tabular}{lcccccc}
\toprule
Model &  BLEU-2 & BLEU-4 & ROUGE-1 & ROUGE-2 & ROUGE-L & METEOR \\
\midrule
Llama2-7B*        & 25.48  & 21.04 & 31.63 & 19.42  & 25.48  & 43.51 \\
Llama2-7B        &  28.15 & 23.24 & 35.14 & 22.08  &  30.41 & 46.87 \\
2D-MoLM        & \underline{30.84} & \underline{25.09} &  \underline{38.46} & \underline{24.22}  & \underline{33.04}  & \underline{50.92} \\
3D-MoLM        &  \textbf{32.00} & \textbf{26.13} & \textbf{40.13}  & \textbf{25.55}  & \textbf{34.64}  & \textbf{52.15} \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Property (\textcolor{teal}{2D} and \textcolor{orange}{3D}) prediction results on the computed property subset of 3D-MoIT.
The MAE with a valid answer rate (\%) is reported -- LMs might generate responses without numerical values.
* denotes official checkpoint without instruct-tuning on 3D-MoIT.
\textbf{Bold} and \underline{underline} indicate the best and the second best performance, respectively.}
\label{tab:instruction-des}
{\setlength{\tabcolsep}{4pt}
\begin{scriptsize}
\begin{tabular}{lcccccccc}
\toprule
Model &\textcolor{teal}{Weight (g/mol)}&\textcolor{teal}{LogP}&\textcolor{teal}{TPSA (\text{\AA}$^2$)}&\textcolor{teal}{Complexity}&\textcolor{orange}{HOMO (eV)}&\textcolor{orange}{LUMO (eV)}&\textcolor{orange}{H-L Gap (eV)}&\textcolor{orange}{SCF ($10^5$eV)}\\
\midrule
Llama2-7B*        & 45.87 (97\%) & 22.18 (98\%) & 23.38 (96\%) & 94.21 (96\%) & 3.15 (72\%)  & 1.19 (79\%) & 2.16 (74\%) & -\\
Llama2-7B        &  18.01 (99\%) & 14.12 (99\%) & 13.21 (99\%) &  72.12 (99\%) & 1.84 (90\%)  & 0.68 (98\%) & 1.62 (98\%) & 0.65 (99\%)\\
2D-MoLM        & 18.53 (99\%) & 13.78 (99\%) &  12.73 (99\%) & 65.32 (99\%)  & 1.80 (93\%)  & 0.63 (99\%) & 1.44 (99\%)&0.67 (99\%)\\
3D-MoLM        & 17.49 (99\%) & 13.29 (99\%) & 12.65 (99\%) & 55.57 (98\%) & 1.06 (92\%) &  0.24 (99\%) & 0.82 (99\%) & 0.26 (99\%)\\
\bottomrule
\end{tabular}
\end{scriptsize}
}
\end{table*}

\begin{table}[t]
\centering
\caption{Cross-modal retrieval results (\%) on PCdes. 
$\dag$ indicates results from~\citep{momu}.
\textbf{Bold} and \underline{underline} indicate the best and the second best performance, respectively.}
\label{tab:cross-modal-retrieval}
 \begin{tabular}{lcccccccc}\toprule
    & \multicolumn{4}{c}{Retrieval in batch} & \multicolumn{4}{c}{Retrieval in test set} \\
    & \multicolumn{2}{c}{M2T (\%)} & \multicolumn{2}{c}{T2M (\%)} & \multicolumn{2}{c}{M2T (\%)} & \multicolumn{2}{c}{T2M (\%)} \\\cmidrule(lr){2-5} \cmidrule(lr){6-9}
   Model & Acc & \multicolumn{1}{c}{R@20} & Acc & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c}{Acc} & R@20 & \multicolumn{1}{c}{Acc} & R@20 \\\midrule
   \multicolumn{2}{l}{\textbf{1D SMILES}} & & \multicolumn{1}{l}{} & & & \multicolumn{1}{l}{} & & \multicolumn{1}{l}{} \\
   Sci-BERT$^\dag$ & 62.6 & - & 61.8 & - & - & 60.7 & - & 60.8 \\
   KV-PLM$^\dag$ & 77.9 & - & 65.0 & - & - & 75.9 & - & 64.3 \\\midrule
   \multicolumn{2}{l}{\textbf{2D Graph}} & & \multicolumn{1}{l}{} & & & \multicolumn{1}{l}{} & & \multicolumn{1}{l}{} \\
   MoMu-S$^\dag$ & 80.6 & - & 77.0 & - & - & 79.1 & - & 75.5 \\
   MoMu-K$^\dag$ & 81.1 & - & 80.2 & - & - & 80.2 & - & 79.0 \\
   3D-MoLM w/o MTM & 88.5 & \multicolumn{1}{c}{97.6} & 88.4 & \multicolumn{1}{c}{97.6} & \multicolumn{1}{c}{59.1} & 88.2 & \multicolumn{1}{c}{59.1} & 87.5 \\
   3D-MoLM & \textbf{89.1} & \multicolumn{1}{c}{\textbf{99.5}} & \textbf{86.5} & \multicolumn{1}{c}{\textbf{98.9}} & \multicolumn{1}{c}{\textbf{59.6}} & \textbf{89.6} & \multicolumn{1}{c}{\textbf{59.8}} & \textbf{87.9} \\\bottomrule
   \end{tabular}
\end{table}
